LIGO-PINN: Learned Initialization via Gated Optimization to Alleviate Convergence Failures in Physics Informed Neural Networks

Physics-informed neural networks (PINNs) have had a broad research impact in modeling domains governed by partial differential equations (PDE). However, PINNs have been shown to perform poorly, sometimes even converging to trivial solutions, in challenging PDE domains, or when generalizing to unseen but related PDE domains. Previously proposed solutions detail hyperparameter tuning to reduce loss imbalance between data-driven and physics guided losses, curriculum learning based training strategies, or dynamic re-sampling of hard collocation points. These methods face certain pitfalls: hyperparameter tuning is expensive, designing a training curriculum is ambiguous in multi-parameter PDE settings, and dynamic resampling still fails in complex PDE settings. Complementary to this line of thinking, we believe the initial PINN network weights also play a crucial role in the emergence of catastrophic failures during training, yet the effect of PINN weight initialization has been surprisingly under-investigated. To this end, we propose a framework for Learned Initialization via Gated Layerwise Optimization (LIGO-PINN) to overcome PINN convergence failures. Through rigorous evaluation on 1D and 2D PDE domains, including a challenging 2D fluid dynamics setting, we demonstrate that our methodology outperforms state-of-the-art methods designed to alleviate PINN failures, achieving a 91.5% average performance improvement across six baselines and 81% over the strongest baseline. We also verify that LIGO-PINN generalizes to 3D unstructured domains. Finally, we analyze training dynamics across all three PDE domains to explain both LIGO-PINN's improvement and the convergence failure of traditional PINNs. Code: https://github.com/scailab/ligo-pinn Keywords: Machine Learning, Physics-Informed Neural Networks, Deep Learning, PDE Modeling

==> sections/c4.ProblemFormulation/mysolution.tex <==
% \subsection{\mymethod{}:\mymethodfull{}}

% Inspired by foundational works in meta‐learning~\citep{finn_model-agnostic_2017} and curriculum learning~\citep{krishnapriyan_characterizing_2021}, we bring together the following key insights to construct a learned‐initialization framework for physics‐informed neural networks:


% \medskip
% \noindent\textbf{Invariance encoding}  
% We begin with a Randomly Initialized weights \(\theta_0\) and pool of \(N\) training tasks \(\{T_i\}_{i=1}^N\).  At each meta‐iteration \(t\):

% \textbf{Task‐specific inner loop:} sample a mini‐batch of \(K\) tasks 
% \(\{T_{i_j}\}_{j=1}^K\sim p(T)\) from the pool, clone \(\theta_t\) for each, and perform
% \[
% \theta'_{t,i_j}
% = \theta_t
% - \eta_{\mathrm{inner}}
% \,\nabla_{\theta}\,
% \mathcal{L}_{T_{i_j}}(\theta_t).
% \]



% Meta Loss across task: All copied model are backpropagation to get get Gradients for meta update
% \[\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)=\sum_{i=1}^K\mathcal{L}_{T_i}(\theta'_{t,i})\]
% % \[
% % \theta_{t+1}
% % = \theta_t
% % - \eta_{\mathrm{outer}}
% % \,\nabla_{\theta}
% % \sum_{i=1}^K
% % \mathcal{L}_{T_i}\bigl(\theta'_{t,i}\bigr).
% % \]






% \medskip
% \noindent\textbf{Gated Layer-wise optimization}  
% A deep network with layers \(l=1,\dots,L\) can be written as 
% \(\hat u_{\Theta}(\mathbf z)=F(\mathbf z;\theta^1,\dots,\theta^L)\), 
% where \(\Theta=(\theta^1,\dots,\theta^L)\).  
% In standard meta learning\cite{finn_model-agnostic_2017}, all layers are optimized simultaneously, without explicit structuring of information flow.  However, deep information propagation theory~\citep{schoenholz2016deep} shows that early layers set the foundation for deeper ones.  Using this insight, we introduce a \emph{Layer Gating Mask} \(g(t)\) that prioritizes learning in initial layers before unblocking deeper ones (see Alg.~\ref{alg:mlayer_iif}, line~\ref{alg:set_g}).

% At each meta‐iteration \(t=0,\dots,T_{\max}-1\), we set the gate for layer \(l\) directly via
% \[
%   g_l(t) =
%   \begin{cases}
%     1, & l \;\le\; \bigl\lfloor\tfrac{t\,L}{T_{\max}}\bigr\rfloor,\\
%     0, & \text{otherwise},
%   \end{cases}
%   \quad l=1,\dots,L.
% \]
% This piecewise schedule starts with only the first layer unlocked and then linearly unblocks deeper layers as training continues, ensuring that early layers focus on learning task‐invariant, general features while later layers specialize to task‐specific mappings—thereby improving overall generalization.


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Proof


% \[
% g(t)=[g^1(t),\,\dots,\,g^L(t)]\in\{0,1\}^L,
% \qquad
% \nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)
% =[\nabla_{\theta^1}\mathcal{L}_{\mathrm{meta}},\,\dots,\,\nabla_{\theta^L}\mathcal{L}_{\mathrm{meta}}],
% \]
% where each \(g^l(t)\) controls the update strength of layer \(l\).  The layer‐wise update is then
% \[
% \theta^{l}_{t+1}
% =\theta^{l}_t
% -\eta_{\mathrm{outer}}\,g^l(t)\,\nabla_{\theta^l}\mathcal{L}_{\mathrm{meta}}(\theta_t),
% \quad l=1,\dots,L,
% \]
% as implemented in Alg.~\ref{alg:mlayer_iif}, line~\ref{alg:outer}.  

% The updated \(\theta_{t+1}\) is then used in the next meta‐iteration, gradually encoding the invariant structure across all sampled PDE tasks.  


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GATE







% \begin{figure}[tb]

%   \centering
%   %─────────────────────────────────────────────────────────
  
%   \begin{minipage}[t]{0.47\textwidth}
%   \small
% \begin{algorithm}[H]
%   \caption{\mymethodfull{}}\label{alg:mlayer_iif}
%   \LinesNumberedHidden
%   \setcounter{AlgoLine}{0}
%   \DontPrintSemicolon
%   \SetAlgoLined
%   \KwIn{Tasks \(p(T)\), initial weights \(\theta_0\), inner LR \(\eta_{\mathrm{inner}}\), outer LR \(\eta_{\mathrm{outer}}\),\\
%          total meta‐iterations \(T_{\max}\), Sampled Task \(k\), inner steps \(inner\)}
%   \KwOut{Meta‐trained \(\theta\)}
%   \For(\tcp*[h]{meta‐iterations \(t=0,\dots,T_{\max}-1\)}){\(t\leftarrow0\)}{
    
%     \nl\label{alg:sample} Sample batch \(\{T_i\}_{i=1}^N\sim p(T)\)\;
%     \For{\(i=1\) \KwTo \(K\)}{
%       \nl\label{alg:inner} \(\theta'_{t,i}\gets\theta_t - \eta_{\mathrm{inner}}\,\nabla_{\theta}\mathcal{L}_{T_i}(\theta_t)\)\;
%     }
%     \nl\label{alg:meta_grad}
%     Compute \(\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
%     \For{\(l=1\) \KwTo \(L\)}{
%     \nl\label{alg:set_g} \(g_l(t)=\mathbf{1}\{l\le\lfloor tL/T_{\max}\rfloor\}\))\;
%       \nl\label{alg:outer} \(\theta^{(l)}_{t+1}\gets\theta^{(l)}_t - \eta_{\mathrm{outer}}\,g_l(t)\,\nabla_{\theta^{(l)}}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
%     }
%   }
% \end{algorithm}



    
%     \subcaption{Meta‐training with layer gating.}
%     \label{fig:alg-meta}
%   \end{minipage}\hfill
%   %─────────────────────────────────────────────────────────
%   \begin{minipage}[t]{0.45\textwidth}
%   \small
% \begin{algorithm}[H]
% \LinesNumberedHidden
% \DontPrintSemicolon
% \SetAlgoLined
% \caption{Fine‐Tuning on New PDE Task}\label{alg:fine_tune}
% \KwIn{Meta‐trained \(\theta_{\mathrm{meta}}\), new task \(T_{\mathrm{new}}\), LR \(\eta_{\mathrm{inner}}\), inner epochs \(E\)}
% \KwOut{Task‐adapted weights \(\theta\)}
% \nl \(\theta \gets \theta_{\mathrm{meta}}\)\;
% \For{\(e=1\) \KwTo \(E\)}{
%   \nl \(\theta \gets \theta - \eta_{\mathrm{inner}}\,\nabla_{\theta}\,\mathcal{L}_{T_{\mathrm{new}}}(\theta)\)\;
% }
% \end{algorithm}
%   \end{minipage}
%   %─────────────────────────────────────────────────────────
%   \caption{(\textbf{a}) Meta‐training stage of LeIn‐PINN with layer gating.  (\textbf{b}) Downstream fine‐tuning on a new PDE task.}
%   \label{fig:algorithms}
% \end{figure}






% \begin{algorithm}[tb]
% \LinesNumbered
% \DontPrintSemicolon
% \SetAlgoLined
% \caption{\mymethodfull{}}\label{alg:mlayer_iif}
% \KwIn{Tasks \(p(T)\), inner LR \(\alpha\), meta LR \(\beta\),\\
%        total iters \(T_{\max}\), tasks per batch \(N\), inner batch size \(K\)}
% \KwOut{Meta‐trained \(\theta\)}
% \nl\label{alg:init} Initialize \(\theta\sim\mathcal{N}(0,\sigma^2I)\)\;
% \nl\label{alg:compute_tau} Compute \(\tau_l=\lceil\frac{l}{L}T_{\max}\rceil\) for \(l=1,\dots,L\)\;
% \For(\tcp*[h]{meta‐iterations}){\(t=0\) \KwTo \(T_{\max}-1\)}{
%   \nl\label{alg:set_g} Set \(g_l(t)=\mathbf{1}\{t\ge\tau_l\}\) for \(l=1,\dots,L\)\;
%   \nl Sample \(\{T_i\}_{i=1}^N\sim p(T)\)\;
%   \For{\(i\leftarrow1\) \KwTo \(N\)}{
%     \nl\label{alg:inner} \(\theta_i'\gets\theta - \alpha\,\nabla_{\theta}\mathcal{L}_{T_i}(\theta)\)\tcp*{inner update}
%   }
%   \nl\label{alg:meta_grad} \(\Delta\theta\gets\nabla_{\theta}\sum_i\mathcal{L}_{T_i}(\theta_i')\)\tcp*{meta gradient}
%   \nl\label{alg:outer} \(\theta\gets\theta - \beta\,(g(t)\odot\Delta\theta)\)\tcp*{gated outer update}
% }
% \end{algorithm}

% \begin{algorithm}[tb]
% \LinesNumbered
% \DontPrintSemicolon
% \SetAlgoLined
% \caption{Fine-Tuning on New PDE Task}\label{alg:fine_tune}
% \KwIn{Meta-trained \(\theta_{\mathrm{meta}}\), new task \(T_{\mathrm{new}}\), LR \(\eta\), epochs \(E\)}
% \KwOut{Task-adapted weights \(\theta\)}
% \nl \(\theta \gets \theta_{\mathrm{meta}}\)\;
% \For{\(e=1\) \KwTo \(E\)}{
%   \nl \(\theta \gets \theta - \eta\,\nabla_{\theta}\,\mathcal{L}_{T_{\mathrm{new}}}(\theta)\)\;
% }
% \end{algorithm}



==> sections/c4.ProblemFormulation/problem_old.tex <==
\section{Background}
\iffalse In this section, we elucidate the technical details about our proposed~\mymethod{} framework (Sec.~\ref{sec:lein_pinn_formulation}) while including minimal necessary background about physics-informed neural networks (PINN) in Sec.~\ref{sec:pinn_background}.\fi 

In line with the original PINN formulation~\citep{raissi2017physicsinformeddeeplearning}, we consider the general PDE system of the form  $\mathcal{F}\bigl(u(\mathbf{ z},t);\gamma\bigr) = f(\mathbf{z},t)$ where $\mathcal{F}$ is a differential operator that represents the  partial differential equation (PDE).
$u(\mathbf{z},t)$ represents the \emph{state} of the system which is the variable of interest to be estimated. 
$\mathbf{z} \in \Omega \subset \mathbb{R}^d$ represents a d-dimensional spatial coordinate in the domain $\Omega$.
$t \in [0,T]$ represents the temporal coordinate where $T$ indicates the  total time over which the PDE dynamics are to be investigated. Further, $\gamma$ is one or a set of PDE parameters governing the system. $f(\mathbf{z},t)$ is a general source term that could represent external forcing or conservation condition (e.g., when $f(\mathbf{z},t) = 0 \,\forall z\in \Omega$; $\forall t \in [0,T]$).  We also represent the boundary conditions as $\mathcal{B}\bigl(u(\mathbf{z},t)\bigr) = g(\mathbf{z},t)$ at boundary points $\mathbf{z}_b \in \partial\Omega$, which also include points at $t = 0$ (i.e., initial condition). By construction, the ground-truth $g(\mathbf{z},t)$ is known for all boundary points in $\partial\Omega$.


Note, in this work, we explore the \emph{forward-modeling problem}  on two separate PDE domains, one (i.e., 1D convection) with a single PDE parameter ($\gamma = \{\beta\}$), $f(\mathbf{z},t) = 0$ and the other, 2D-Helmholtz with two PDE parameters ($\gamma = \{a_1, a_2\}$) and a non-zero forcing function $f(\mathbf{z},t)$. Further details about these domains are included in appendix ~\ref{sec:dataset_desc}.


\subsection{Physics-Informed Neural Networks (PINN)}\label{sec:pinn_background}
\iffalse 
and the goal is to learn the solution $u(\mathbf z)$ at all points $z \in \Omega$. and its boundary conditions:
\begin{equation}
  \mathcal{F}\bigl(u(\mathbf z);\gamma\bigr) = f(\mathbf z),
  \quad
  \mathbf z \in \Omega \subset \mathbb{R}^{d+1},
  \quad
  \mathcal{B}\bigl(u(\mathbf z)\bigr) = g(\mathbf z),
  \quad
  \mathbf z \in \partial\Omega.
\end{equation}
\fi 
The primary goal of PINNs is to train a neural network governed by a set of parameters $\Theta$, which when conditioned on a domain coordinate $(\mathbf{z},t)$, is capable of estimating $\hat{u}(\mathbf{z},t) \in \mathbb{R}$, such that it closely approximates $u(\mathbf{z},t) \in  \mathbb{R} \,\forall \mathbf{z} \in \Omega$ (i.e., internal domain points), $\mathbf{z}_b \in \partial\Omega$ (initial and boundary points).  For ease of notation, let us represent as $\hat{u}_\Theta(\mathbf{z},t)$, the prediction yielded by the PINN at point $(\mathbf{z},t)$ governed by parameters $\Theta$. Then the PINN is trained by minimizing the objective in Eq.~\ref{eq:pinn_optim_obj} where $\mathcal{L}(\Theta)$ is a composite loss represented in Eq.~\ref{eq:pinn_total_loss}.

 \begin{equation}
\Theta^*=\arg\min_{\Theta}\mathcal{L}(\theta)
\label{eq:pinn_optim_obj}
 \end{equation}
 
In Eq.~\ref{eq:pinn_total_loss}, the first term indicates the \emph{residual} (or physics-informed) loss which is applied at the non-boundary (i.e., internal) points of the domain $\Omega$ and directly ensures consistency of the predictions yielded by the PINN with the governing PDE at these points. 

\begin{equation}
  \mathcal{L}(\Theta)
  = \lambda_r \frac{1}{N_{\Omega}} \sum_{i=1}^{N_{\Omega}} \bigl|\mathcal{F}(\hat u_{\Theta}(\mathbf{z}_i,t_i);\gamma)-f(\mathbf{z}_i,t_i)\bigr|^2
  + \frac{1}{N_{\partial\Omega}} \sum_{j=1}^{N_{\partial\Omega}} \bigl|\mathcal{B}(\hat u_{\Theta}(\mathbf{z}_j,t_j))-g(\mathbf{z}_j,t_j)\bigr|^2
  \label{eq:pinn_total_loss}
\end{equation}

On the other hand, the second term is a data driven (e.g., MSE) loss and is only applied at the boundary $\partial\Omega$, where ground-truth values are known. The optimization of Eq.~\ref{eq:pinn_total_loss} proceeds by sampling (randomly or otherwise) a set of $N_\Omega$  domain co-ordinates from $\Omega$ (called \emph{collocation} points) as well as $N_{\partial\Omega}$ boundary coordinates from $\partial\Omega$. $\lambda_r$ is a hyperparameter that
 governs the effect of the physics-informed, (i.e., residual) loss during PINN training.
 \iffalse 
The PINN is then trained (according to objective in Eq.~\ref{eq:pinn_optim_obj}) to minimize the residual loss (only applied at sampled collocation points) and data-driven loss (only applied at boundary points).\fi  

\iffalse $\mathbf z=[x_1,\dots,x_d,t]\in\mathbb{R}^{d+1}$ is the space--time coordinate; $\Omega$ the computational domain with boundary $\partial\Omega$; $\gamma$ the physical parameters; $f,g$ the forcing and boundary data; \fi 

\section{Problem Formulation}\label{sec:lein_pinn_formulation}
% \subsection{\mymethod{}:\mymethodfull{}}\label{sec:lein_pinn_formulation}
Although the PINN formulation outlined in Eq.~\ref{eq:pinn_optim_obj} and Eq.~\ref{eq:pinn_total_loss} has been highly impactful in solving \emph{forward} problems across variegated PDE  domains, it has recently been found that PINNs fail to learn faithful solutions (and converge to trivial solutions) in challenging (e.g., stiff) PDE contexts. Previous works~\citep{wang2021understanding} have characterized the conflicting and imbalanced gradients between the two loss terms in $\mathcal{L}(\Theta)$ as one of the reasons for such failures. Recent approaches  have proposed solutions to counter such PINN convergence failures by intelligent re-sampling ~\citep{daw_mitigating_2023} and curriculum based PINN training~\citep{krishnapriyan_characterizing_2021} training. 

Complementary to these works, we hypothesize that PINN convergence failures in \emph{challenging} (a.k.a. hard) PDE domains, can be alleviated, if the weights $\Theta$ of the PINN, instead of being randomly initialized, are \underline{systematically initialized} prior to training on the \emph{hard} domain. To this end, we propose a \emph{Learned-Initialization} (LeIn) mechanism to systematically learn better initial weights for PINNs such that PINNs trained with LeIn weights do not experience catastrophic failures in challenging PDE domains. Our proposed LeIn approach comprises of two facets (i) Invariance Encoding (ii) Gated Layer-wise Optimization. 

\textbf{Invariance Encoding (IE).} If the goal of the PINN is to learn a challenging PDE domain governed by PDE parameter $\gamma_{\mathrm{hard}}$, IE seeks to first train a randomly initialized PINN model on a set of \emph{relatively easier} configurations of the PDE with parameters $\Gamma_{\mathrm{easy}} = \{\gamma_{1},\dots,\gamma_{K}\}$ to enable a distillation of the \emph{invariant} physics across $\Gamma_{\mathrm{easy}}$. Our approach for IE is grounded in  foundational works of meta‐learning~\citep{finn_model-agnostic_2017}.  IE begins with randomly initialized \emph{global} PINN weights \(\Theta_0\) and pool of $K$ tasks in $\Gamma_{\mathrm{easy}}$.
The IE learning process is carried out for $\mathcal{R}$ iterations $\{1,2,\dots,\mathcal{R}\}$ and at each training iteration $r$, tasks $\{\mathcal{T}_1,\dots,\mathcal{T}_k\}$ are randomly sampled from the task distribution $p(\Gamma_{\mathrm{easy}})$ of easy tasks and $k$ identical copies $\{\Theta'_{r,1},\dots,\Theta'_{r,k}\}$ of the current global PINN weights $\Theta_r$ are created. Each $\Theta'_{r,i}$ proceeds to be optimized (via. gradient descent) employing data from task $\mathcal{T}_i$ at iteration $r$ for `J' \emph{inner} iterations (for simplicity we assume `J' = 1). Let $\Theta''_{r,i}$ represent the updated version of $\Theta'_{r,i}$ after `J' inner gradient-descent update iterations.  
The \emph{common} representations across all $k$  task models $\{\Theta''_{r,1},\dots,\Theta''_{r,k}\}$ are distilled into $\Theta_r$ via. a `meta-update' as indicated in Eq.~\ref{eq:meta_update} where $\mathcal{L}_{\mathcal{T}_i}(\Theta''_{r,i})$ represents the loss in Eq.~\ref{eq:pinn_total_loss} calculated w.r.t parameters $\Theta''_{r,i}$ with data from task $\mathcal{T}_i$ and $\eta_{\mathrm{outer}}$ represents the learning rate.

\begin{align}
\begin{split}
\nabla_{\Theta_r}\mathcal{L}_{\mathrm{meta}}^r &=\nabla_{\Theta_r}\sum_{i=1}^k\mathcal{L}_{\mathcal{T}_i}(\Theta''_{r,i})\\
\Theta_{r+1} &= \Theta_{r} - \eta_{\mathrm{outer}}\nabla_{\Theta_r}\mathcal{L}_{\mathrm{meta}}^r 
\label{eq:meta_update}
\end{split}
\end{align}

 

\iffalse 
On each task $\{\mathcal{T}_i\}_{i=1}^k$

At each iteration \(t\):

Task‐specific inner loop: Sample a mini‐batch of \(K\) tasks 
\(\{T_{i}\}_{i=1}^K\sim p(T)\) from the pool, clone \(\theta_t\) for each task and optimize using gradient descent
\[
\theta'_{t,i_j}
= \theta_t
- \eta_{\mathrm{inner}}
\,\nabla_{\theta}\,
\mathcal{L}_{T_{i_j}}(\theta_t).
\]


Meta Loss across task: Backpropagate through the all task models to obtain the gradients for updating shared meta weights
\[\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)=\sum_{i=1}^K\mathcal{L}_{T_i}(\theta'_{t,i})\]
% \[
% \theta_{t+1}
% = \theta_t
% - \eta_{\mathrm{outer}}
% \,\nabla_{\theta}
% \sum_{i=1}^K
% \mathcal{L}_{T_i}\bigl(\theta'_{t,i}\bigr).
% \]

\fi 

\noindent\textbf{Gated Layer-wise optimization (GLO).} Traditional meta-learning approaches~\citep{finn_model-agnostic_2017,rajeswaran2019meta} are not physics-informed and treat all tasks in $\Gamma_{\mathrm{easy}}$ as resulting in similar training dynamics (which is why the meta-update in Eq.~\ref{eq:meta_update} is a simple summation of all task gradients. Further, the non-trivial dynamics between the physics-based residual loss and the data-driven loss also affects different layers in the neural network differently~\citep{wang2021understanding}. To address these gaps that manifest uniquely in the physics-informed PDE modeling context, we augment the IE procedure with the GLO mechanism by introducing a \emph{gated} update of layers during each meta-update, such that a gating mechanism $g(r)$, \emph{unlocks} deeper layers, exposing their parameters to gradient-based optimization, gradually, over the training iterations from 1 to $\mathcal{R}$.  

\textcolor{red}{bookmark}

A deep network with layers \(l=1,\dots,L\) can be written as 
\(\hat u_{\Theta}(\mathbf z)=F(\mathbf z;\theta^1,\dots,\theta^L)\), 
where \(\Theta=(\theta^1,\dots,\theta^L)\).  
In standard meta-learning\cite{finn_model-agnostic_2017}, all layers of $\Theta_r$ are optimized simultaneously, without explicit structuring of information flow.  However, deep information propagation theory~\citep{schoenholz2016deep} shows that early layers set the foundation for deeper ones.  Using this insight, we introduce a \emph{Layer Gating Mask} \(g(r)\) that prioritizes learning in initial layers before unmasking deeper ones (see Alg.~\ref{alg:mlayer_iif}, line~\ref{alg:set_g}).

At each outer‐iteration \(r \in \{1,2,\dots,\mathcal{R}\}\), the (binary) gating value for layer \(l\) is calculated via. a linear gating mechanism
\[
  g_l(r) =
  \begin{cases}
    1, & l \;\le\; \bigl\lfloor\tfrac{r\,L}{\mathcal{R}}\bigr\rfloor,\\
    0, & \text{otherwise},
  \end{cases}
  \quad l=1,\dots,L.
\]
The gating schedule begins with the first layer unmasked, followed by linear unmasking of deeper layers as training progresses, ensuring localized (and thereby more manageable) effects of non-trivial loss dynamics.  
\iffalse This ensures  early layers focus on learning task‐invariant, general features while later layers specialize to task‐specific mappings—thereby, improving overall generalization.\fi 
Although the proposed $g(r)$ function is linear, GLO can easily admit any general gating mechanism.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Proof

\[
g(t)=[g_1(t),\,\dots,\,g_L(t)]\in\{0,1\}^L,
\qquad
\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)
=[\nabla_{\theta^1}\mathcal{L}_{\mathrm{meta}},\,\dots,\,\nabla_{\theta^L}\mathcal{L}_{\mathrm{meta}}],
\]
where each \(g_l(t)\) controls the update strength of layer \(l\).  The layer‐wise update is then
\[
\theta^{l}_{t+1}
=\theta^{l}_t
-\eta_{\mathrm{outer}}\,g^l(t)\,\nabla_{\theta^l}\mathcal{L}_{\mathrm{meta}}(\theta_t),
\quad l=1,\dots,L,
\]
as implemented in Alg.~\ref{alg:mlayer_iif}, line~\ref{alg:outer}.  

The updated \(\theta_{t+1}\) is then used in the next meta‐iteration, gradually encoding the invariant structure across all sampled PDE tasks.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GATE

\begin{algorithm}[!ht]
  \caption{\mymethodfull{} }\label{alg:mlayer_iif}
  \LinesNumberedHidden
  \setcounter{AlgoLine}{0}
  \DontPrintSemicolon
  \SetAlgoLined
  \KwIn{Tasks \(p(T)\), initial weights \(\theta_0\), inner LR \(\eta_{\mathrm{inner}}\), outer LR \(\eta_{\mathrm{outer}}\),\\
         total meta‐iterations \(T_{\max}\), Sampled Task \(k\), inner steps \(inner\)}
  \KwOut{Meta‐trained \(\theta\)}
  \For(\tcp*[h]{meta‐iterations \(t=0,\dots,T_{\max}-1\)}){\(t\leftarrow0\)}{
    
    \nl\label{alg:sample} Sample batch \(\{T_i\}_{i=1}^N\sim p(T)\)\;
    \For{\(i=1\) \KwTo \(K\)}{
      \nl\label{alg:inner} \(\theta'_{t,i}\gets\theta_t - \eta_{\mathrm{inner}}\,\nabla_{\theta}\mathcal{L}_{T_i}(\theta_t)\)\;
    }
    \nl\label{alg:meta_grad}
    Compute \(\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
    \For{\(l=1\) \KwTo \(L\)}{
    \nl\label{alg:set_g} \(g_l(t)=\mathbf{1}\{l\le\lfloor tL/T_{\max}\rfloor\}\))\;
      \nl\label{alg:outer} \(\theta^{(l)}_{t+1}\gets\theta^{(l)}_t - \eta_{\mathrm{outer}}\,g_l(t)\,\nabla_{\theta^{(l)}}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
    }
  }
\end{algorithm}


\begin{algorithm}[!ht]
\LinesNumberedHidden
\DontPrintSemicolon
\SetAlgoLined
\caption{Fine‐Tuning on New PDE Task}\label{alg:fine_tune}
\KwIn{Meta‐trained \(\theta_{\mathrm{meta}}\), new task \(T_{\mathrm{new}}\), LR \(\eta_{\mathrm{inner}}\), inner epochs \(E\)}
\KwOut{Task‐adapted weights \(\theta\)}
\nl \(\theta \gets \theta_{\mathrm{meta}}\)\;
\For{\(e=1\) \KwTo \(E\)}{
  \nl \(\theta \gets \theta - \eta_{\mathrm{inner}}\,\nabla_{\theta}\,\mathcal{L}_{T_{\mathrm{new}}}(\theta)\)\;
}
\end{algorithm}




%   %─────────────────────────────────────────────────────────
  
% \begin{minipage}{0.45\textwidth}
% \begin{algorithm}[H]
%   \caption{\mymethodfull{} }\label{alg:mlayer_iif}
%   \LinesNumberedHidden
%   \setcounter{AlgoLine}{0}
%   \DontPrintSemicolon
%   \SetAlgoLined
%   \KwIn{Tasks \(p(T)\), initial weights \(\theta_0\), inner LR \(\eta_{\mathrm{inner}}\), outer LR \(\eta_{\mathrm{outer}}\),\\
%          total meta‐iterations \(T_{\max}\), Sampled Task \(k\), inner steps \(inner\)}
%   \KwOut{Meta‐trained \(\theta\)}
%   \For(\tcp*[h]{meta‐iterations \(t=0,\dots,T_{\max}-1\)}){\(t\leftarrow0\)}{
    
%     \nl\label{alg:sample} Sample batch \(\{T_i\}_{i=1}^N\sim p(T)\)\;
%     \For{\(i=1\) \KwTo \(K\)}{
%       \nl\label{alg:inner} \(\theta'_{t,i}\gets\theta_t - \eta_{\mathrm{inner}}\,\nabla_{\theta}\mathcal{L}_{T_i}(\theta_t)\)\;
%     }
%     \nl\label{alg:meta_grad}
%     Compute \(\nabla_{\theta}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
%     \For{\(l=1\) \KwTo \(L\)}{
%     \nl\label{alg:set_g} \(g_l(t)=\mathbf{1}\{l\le\lfloor tL/T_{\max}\rfloor\}\))\;
%       \nl\label{alg:outer} \(\theta^{(l)}_{t+1}\gets\theta^{(l)}_t - \eta_{\mathrm{outer}}\,g_l(t)\,\nabla_{\theta^{(l)}}\mathcal{L}_{\mathrm{meta}}(\theta_t)\)\;
%     }
%   }
% \end{algorithm}


    
%   \end{minipage}\hfill

  
%   %─────────────────────────────────────────────────────────
% \begin{minipage}{0.45\textwidth}
% \begin{algorithm}[H]\label{fig:alg-meta}
% \LinesNumberedHidden
% \DontPrintSemicolon
% \SetAlgoLined
% \caption{Fine‐Tuning on New PDE Task}\label{alg:fine_tune}
% \KwIn{Meta‐trained \(\theta_{\mathrm{meta}}\), new task \(T_{\mathrm{new}}\), LR \(\eta_{\mathrm{inner}}\), inner epochs \(E\)}
% \KwOut{Task‐adapted weights \(\theta\)}
% \nl \(\theta \gets \theta_{\mathrm{meta}}\)\;
% \For{\(e=1\) \KwTo \(E\)}{
%   \nl \(\theta \gets \theta - \eta_{\mathrm{inner}}\,\nabla_{\theta}\,\mathcal{L}_{T_{\mathrm{new}}}(\theta)\)\;
% }
% \end{algorithm}
% \end{minipage}




% \FloatBarrier


% \begin{minipage}[t]{0.48\textwidth}
%   % declare the float type so captions number correctly
%   \captionsetup{type=algorithm}  
%   \captionof{algorithm}{\mymethodfull{}}\label{alg:mlayer_iif}
%   \begin{algorithmic}[1]
%     \State \textbf{Input:} tasks $p(T)$, init $\theta_0$, inner LR $\eta_{\rm inner}$, outer LR $\eta_{\rm outer}$, \dots
%     \State \textbf{Output:} meta‐trained $\theta$
%     \For{$t=0,\dots,T_{\max}-1$}
%       \State sample batch $\{T_i\}\sim p(T)$  
%       \For{$i=1\dots K$}
%         \State $\theta'_{t,i}\gets\theta_t - \eta_{\rm inner}\,\nabla_\theta \mathcal{L}_{T_i}(\theta_t)$
%       \EndFor
%       \State compute $\nabla_\theta \mathcal{L}_{\rm meta}(\theta_t)$
%       \For{$l=1\dots L$}
%         \State $g_l(t)\gets\mathbf{1}\{l\le\lfloor tL/T_{\max}\rfloor\}$  
%         \State $\theta^{(l)}_{t+1}\gets\theta^{(l)}_t - \eta_{\rm outer}\,g_l(t)\,\nabla_{\theta^{(l)}}\mathcal{L}_{\rm meta}(\theta_t)$
%       \EndFor
%     \EndFor
%   \end{algorithmic}
% \end{minipage}\hfill
% \begin{minipage}[t]{0.48\textwidth}
%   \captionsetup{type=algorithm}
%   \captionof{algorithm}{Fine‐Tuning on New PDE Task}\label{alg:fine_tune}
%   \begin{algorithmic}[1]
%     \State \textbf{Input:} meta‐trained $\theta_{\rm meta}$, new task $T_{\rm new}$, LR $\eta_{\rm inner}$, epochs $E$
%     \State \textbf{Output:} task‐adapted $\theta$
%     \State $\theta\gets\theta_{\rm meta}$
%     \For{$e=1\dots E$}
%       \State $\theta\gets\theta - \eta_{\rm inner}\,\nabla_\theta \mathcal{L}_{T_{\rm new}}(\theta)$
%     \EndFor
%   \end{algorithmic}
% \end{minipage}

\subsection{Experimental Setup}
To validate our approach, we compare \mymethod{} against a suite of established PINN variants; the full descriptions of these baselines can be found in Appendix~\ref{sec:model_explain}, and the complete details of our experimental setup—including PDE definitions, network architectures, training procedures, and hyperparameter selections—are provided in Appendix~\ref{appen:exp-setup-heat1d} and \ref{appen:exp-setup-helm2d}. We refer the reader to these appendices for all implementation specifics and additional evaluation protocols underlying the results presented here.


==> sections/c6.ResultsAnalysis/ns_table_combined.tex <==

\iffalse 
\begin{table}[!ht]
\small
\setlength{\tabcolsep}{5pt}
\caption{Forward problem: Pressure ($p$) prediction errors across Reynolds numbers. Lowest values in each column are in bold.}
\label{tab:ns_forward}
\centering
\begin{tabular}{lccc|c}
\toprule
\multirow{\textbf{Method} & 600 & 800 & 1000 & Avg.\\}
\midrule
\methodpinnf
& 0.0183
& 0.1934
& 0.0257
& 0.0791 \\

\methodpinnd~\citep{wang2021understanding}
& 0.0239
& 0.0958
& 0.0353
& 0.0517 \\

\methodcurriculumn~\citep{krishnapriyan_characterizing_2021}
& 0.3011
& 0.2597
& 0.2309
& 0.2639 \\

\methodevo~\citep{daw_mitigating_2023}
& 0.3519
& 0.4966
& 0.2620
& 0.3702 \\

\methodmetapde~\citep{qin2022metapdelearningsolvepdes}
& 0.3172
& 0.2997
& 0.2812
& 0.2994 \\

\methodhyperlr
& 0.2155
& 0.1253
& 0.1910
& 0.1773 \\

\textbf{\mymethod{} (Ours)}
& \textbf{0.0051}
& \textbf{0.0379}
& \textbf{0.0077}
& \textbf{0.0169} \\
\bottomrule
\end{tabular}

\setlength{\tabcolsep}{3pt}
\caption{Navier--Stokes: $\lambda_{\mathrm{adv}}$ and $\lambda_{\mathrm{visc}}$ estimation errors across Reynolds numbers. Lowest values in each column are in bold.}
\label{tab:ns_inverse}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{3}{cc}|cc}
\toprule
\textbf{Method}
 & \multicolumn{2}{c}{\textbf{Re\_600}}
 & \multicolumn{2}{c}{\textbf{Re\_800}}
 & \multicolumn{2}{c}{\textbf{Re\_1000}}
 & \multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$ \\
\midrule

\methodpinnf
 & 0.1212 & 0.0282
 & 0.1210 & 0.0441
 & \textbf{0.0191} & \textbf{0.0074}
 & 0.0871 & 0.0266 \\

\methodpinnd~\citep{wang2021understanding}
 & 0.0472 & 0.0085
 & 0.1539 & 0.0370
 & 0.0478 & \textbf{0.0074}
 & 0.0830 & 0.0176 \\

\methodcurriculumn~\citep{krishnapriyan_characterizing_2021}
 & 0.6251 & 0.1645
 & 0.7021 & 0.1479
 & 0.6380 & 0.1787
 & 0.6551 & 0.1637 \\

\methodevo~\citep{daw_mitigating_2023}
 & 0.3841 & 0.0692
 & 0.5106 & 0.0722
 & 0.2222 & 0.1189
 & 0.3723 & 0.0868 \\

\methodmetapde~\citep{qin2022metapdelearningsolvepdes}
 & 0.4320 & 0.1312
 & 0.6910 & 0.2979
 & 0.6910 & 0.2370
 & 0.6046 & 0.2220 \\

\methodhyperlr
 & 0.0509 & 0.0108
 & \textbf{0.0633} & 0.0133
 & 0.1162 & 0.0163
 & 0.0768 & 0.0135 \\

\textbf{\mymethod{} (Ours)}
 & \textbf{0.0083} & \textbf{0.0068}
 & 0.0682 & \textbf{0.0081}
 & 0.2194 & 0.0253
 & \textbf{0.0986} & \textbf{0.0134} \\
\bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[!ht]
\small
\setlength{\tabcolsep}{3pt}
\caption{Navier--Stokes: $\lambda_{\mathrm{adv}}$ and $\lambda_{\mathrm{visc}}$ estimation errors across Reynolds numbers. Lowest values in each column are in bold.}
\label{tab:ns_inverse}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{3}{cc}|cc}
\toprule
\textbf{Method}
 & \multicolumn{2}{c}{\textbf{Re\_600}}
 & \multicolumn{2}{c}{\textbf{Re\_800}}
 & \multicolumn{2}{c}{\textbf{Re\_1000}}
 & \multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$
 & $\lambda_{\mathrm{adv}}$ & $\lambda_{\mathrm{visc}}$ \\
\midrule

\methodpinnf
 & 0.1212 & 0.0282
 & 0.1210 & 0.0441
 & \textbf{0.0191} & \textbf{0.0074}
 & 0.0871 & 0.0266 \\

\methodpinnd~\citep{wang2021understanding}
 & 0.0472 & 0.0085
 & 0.1539 & 0.0370
 & 0.0478 & \textbf{0.0074}
 & 0.0830 & 0.0176 \\

\methodcurriculumn~\citep{krishnapriyan_characterizing_2021}
 & 0.6251 & 0.1645
 & 0.7021 & 0.1479
 & 0.6380 & 0.1787
 & 0.6551 & 0.1637 \\

\methodevo~\citep{daw_mitigating_2023}
 & 0.3841 & 0.0692
 & 0.5106 & 0.0722
 & 0.2222 & 0.1189
 & 0.3723 & 0.0868 \\

\methodmetapde~\citep{qin2022metapdelearningsolvepdes}
 & 0.4320 & 0.1312
 & 0.6910 & 0.2979
 & 0.6910 & 0.2370
 & 0.6046 & 0.2220 \\

\methodhyperlr
 & 0.0509 & 0.0108
 & \textbf{0.0633} & 0.0133
 & 0.1162 & 0.0163
 & 0.0768 & 0.0135 \\

\textbf{\mymethod{} (Ours)}
 & \textbf{0.0083} & \textbf{0.0068}
 & 0.0682 & \textbf{0.0081}
 & 0.2194 & 0.0253
 & \textbf{0.0986} & \textbf{0.0134} \\
\bottomrule
\end{tabular}%
}
\end{table}
\fi 

==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our results and discussion and supplemental results included in appendix are all aligned with claims made with abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:\answerYes{}
    \item[] Justification: We have discussed the limitations of the proposed \mymethod{} approach in Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:\answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification:\hide{\textcolor{red}{In Appendix~\ref{appendix:experimental-setup} we have described the 1D Convection and 2D helmholtz dataset as well as baseline models employed for experimental evaluation. Further, Appendix~\ref{appendix:experimental-setup} also includes exact model architecture and training details for each dataset to facilitate experiment reproducibility.}}
    We have made efforts to ensure that our results are reproducible. Specifically, our contribution is a specific model for improved training of PINNs in challenging PDE domains. The main text provides a clear description of our proposed \mymethod{} model with evaluation results and discussion. Further, to ensure experiment reproducibility, we have included in Appendix~\ref{appendix:experimental-setup}, the full architecture of our model along with training and optimization configurations as well as detailed experimental setups for each evaluation PDE domain. Finally, we have provided our code including experiment scripts, to enable full reproducibility of all reported results and figures in the paper.\hide{Additional implementation details, including architecture specifications, hyperparameters, and training schedules, are provided in the Appendix~\ref{appen:exp-setup-conv1d}.} As the full datasets are too large to share directly, we instead provide dataset generation code.\hide{We also include experiment scripts, along with the PINN implementation, to allow reproduction of all reported results and figures using our methodology.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have provided code as part of supplementary material and code includes README files with instructions to reproduce results from paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{appen:exp-setup-conv1d}includes exact model architecture and training details for each of the three datasets used in our experimental evaluations to help understand the result.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have run all our experimental evaluations multiple time across training runs (i.e.,5 times with different random seeds) and reported a mean and standard deviation. Although the main paper due to space constraints, only includes the mean values of each evaluation experiment, each table in the main paper has a corresponding table in Appendix~\ref{appen:baseline_tables} reporting both mean and standard deviations of each evaluation experiment. Further our percentage improvement results consistent across 5 runs clearly demonstrate significant and persistent performance improvement of \mymethod{} over ALL state-of-the-art PINN baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: In Appendix~\ref{appendix:computation-resource} we detail the compute resources by enumerating the hardware and software resources employed as well as the running time and peak memory usage required for \mymethod{} training.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes this research conforms to NeurIPS Code of Ethics
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification:This work focuses on foundational optimization methods for PDE-based machine learning systems and does not have direct societal impact considerations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    \item[] Justification:
    We acknowledge the use of a large language model (LLM)-based writing assistant for language editing, clarity improvement, and consistency checks of reported numerical summaries. The authors reviewed and verified all LLM-assisted edits, calculations, interpretations, and conclusions. The scientific content, experimental design, results, and final manuscript remain the sole responsibility of the authors.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> sections/introduction.tex <==
\chapter{Introduction}

Machine learning models have increasingly become the preferred choice over traditional computational methods, owing to their ability to model complex patterns and dynamics across diverse domains~\cite{karpatne2017theoryguidedkgml,karpatne2022knowledgekgmlbook}. These models have been applied extensively, from understanding galaxies and climate systems to predicting stock market trends. Wherever data is abundant, machine learning finds its utility. However, the prevalent purely data-driven nature of many machine learning models has raised concerns about interpretability and generalizability. Unlike traditional scientific methodologies, which fundamentally aim to enhance our understanding of natural systems, purely data-driven models if not trained with \emph{representative} datasets often lack insights into the underlying principles governing the data.

\section{Knowledge-Guided Machine Learning}

To address these challenges, Knowledge-Guided Machine Learning (KGML)~\cite{karpatne2017theoryguidedkgml,muralidhardann2018} has emerged as a promising paradigm. KGML integrates domain knowledge / structured information about the problem into the learning process. This enables models to operate more efficiently in data-scarce environments. By constraining the solution space to physically plausible outcomes, KGML mitigates the curse of dimensionality, accelerates convergence, and improves generalization. This domain-driven inductive bias fosters interpretability and ensures solutions adhere to known scientific principles, enhancing their reliability.

\section{Physics-Informed Neural Networks}

Since Newton’s formulation of a mathematical framework~\cite{newton1934principia} using calculus to describe the laws of the universe, humans have relied on principles such as conservation laws and invariants to model and understand physical phenomena. These principles impose remarkable constraints that define both the state and evolution of physical systems~\cite{hill1951hamilton}. Inspired by the rigor of these foundational laws, a significant innovation in scientific machine learning emerged: Physics-Informed Neural Networks (PINNs)~\cite{raissi_physics_2017}. PINNs leverage known physical laws as a form of regularization, seamlessly embedding them into the neural network's loss function to solve both forward and inverse problems~\cite{raissi_physics_2017,raissi2017physicspart1,raissi2018deephiddenphysics,raissi2018numerical} in domains governed by partial differential equations (PDE). 

This paradigm shift has demonstrated remarkable success in tackling complex engineering problems~\cite{chen2020physics,jin2021nsfnets}, particularly in scenarios with limited or noisy data. By integrating physical laws, PINNs adhere closely to underlying system dynamics, enabling robust solutions under challenging conditions for both forward and inverse problems. PINNs have already been successfully applied across a wide range of scientific domains, including geophysics~\cite{yang2021revisit,voytan2020wave}, climate modeling~\cite{lutjens2021pce}, materials science~\cite{shao2020pinn,lin2022development}, and fluid dynamics~\cite{rao2020physics,zhu2021machine}. They have also proven valuable in medical imaging~\cite{van2022physics,sahli2020physics}.
\section{Motivation}

Despite their demonstrated potential, PINNs face notable challenges. One critical issue is the imbalance in the loss function, which often hinders optimization~\cite{wang2021understanding}. Researchers have explored various avenues to address these limitations. For instance, Fourier decomposition methods have been employed to identify failures caused by high-frequency features~\cite{wang2021eigenvector}, while insights from the neural tangent kernel (NTK) perspective have provided a deeper understanding of optimization dynamics~\cite{wang2022and}. Another study~\cite{krishnapriyan_characterizing_2021} revealed that high values of PDE parameters exacerbate PINN failures in predictable ways, shedding light on their limitations and proposing innovative solutions.

Motivated by~\cite{schoenholz2016deep,poole_exponential_2016}, it was empirically shown that traditional neural network initialization schemes like Xavier and Kaiming initialization\cite{glorot2010understanding}, are not the most efficient, and initialization dictates the training bounds.
In line with this thought process, this work proposes an pretraining framework that incorporates invariance from related task to overcome the  failure modes of PINNs in challenging PDE domains. Specifically, our framework grounded in the popular meta-learning paradigm~\cite{finn_model-agnostic_2017} adopts a complementary approach relative to previous efforts~\cite{daw_mitigating_2023,krishnapriyan_characterizing_2021} in overcoming PINN failure modes. Our experimental results also showcase that our proposed method ~\mymethod{} allows the our model to converge to lower magnitude of error for related complex task.

\iffalse I realized that there was less attention on initialization and more on optimization. We know empirically that neural networks are very expressive. I tried to explore the meta-learning framework, in particular, Model-Agnostic Meta-Learning (MAML)~\cite{finn_model-agnostic_2017}, to show that pretraining of related tasks results in a better initialization for our model to adapt better to unseen tasks and avoids the failure modes that plague PINNs. We propose a novel architecture that helps the model meta-learn better for varied tasks.
\fi 

\section{Contributions}

\begin{enumerate}
    \item We propose a novel informed pre-training based solution to overcome catastrophic failures in PINNs.
    \item Our proposed ~\mymethodfull{} (~\mymethod{}) model comprises a novel layer-wise training schedule to effectively alleviate gradient imbalances prevalent in PINN training dynamics.
    \item Through rigorous comparisons with state of the art baseline models, we demonstrate the empirical superiority of our proposed  ~\mymethod{} and provide a qualitative analysis to explain the performance improvement. 
\end{enumerate}
